Signal-Adaptive and Perceptually Optimized Sound Zones with Variable Span Trade-Off Filters

Creating sound zones has been an active research field since the idea was first proposed. So far, most sound zone control methods rely on either an optimization of physical metrics such as acoustic contrast and signal distortion or a mode decomposition of the desired sound field. By using these types of methods, approximately 15 dB of acoustic contrast between the reproduced sound field in the target zone and its leakage to other zone(s) has been reported in practical set-ups, but this is typically not high enough to satisfy the people inside the zones. In this paper, we propose a sound zone control method shaping the leakage errors so that they are as inaudible as possible for a given acoustic contrast. The shaping of the leakage errors is performed by taking the time-varying input signal characteristics and the human auditory system into account when the loudspeaker control filters are calculated. We show how this shaping can be performed using variable span trade-off filters, and we show theoretically how these filters can be used for trading signal distortion in the target zone for acoustic contrast. The proposed method is evaluated based on physical metrics such as acoustic contrast and perceptual metrics such as STOI. The computational complexity and processing time of the proposed method for different system set-ups are also investigated. Lastly, the results of a MUSHRA listening test are reported. The test results show that the proposed method provides more than 20% perceptual improvement compared to existing sound zone control methods.

==> chapters/04_simulations/ch4_0_sub1_sim1_anechoic.tex <==
\begin{figure*}[t]
	\centering
	\captionsetup[subfigure]{justification=centering}
		\subfloat[]{\includegraphics[width=5.8cm]{data/anechoic/sim1_free/fig_AC_(dB)_anechoic_pointwise.png}\label{subfig:ac_free}}\quad
		\subfloat[]{\includegraphics[width=5.8cm]{data/anechoic/sim1_free/fig_nSDP_(dB)_anechoic_pointwise.png}\label{subfig:sdp_free}}\quad
		\subfloat[]{\includegraphics[width=5.8cm]{data/anechoic/sim1_free/fig_TIR_(dB)_anechoic_pointwise.png}\label{subfig:tir_free}}%\hfill
		
		\subfloat[]{\includegraphics[width=5.8cm]{data/anechoic/sim1_free/fig_STOI_anechoic_pointwise.png}\label{subfig:stoi_free}}\quad
		\subfloat[]{\includegraphics[width=5.8cm]{data/anechoic/sim1_free/fig_PSMt_anechoic_pointwise.png}\label{subfig:psmt_free}}\par
		\caption{The mean values (crosses) and the $95\%$ confidence intervals (solid lines) of the performance evaluation metrics in anechoic environment: physical metrics of \protect\subref{subfig:ac_free} AC in dB, \protect\subref{subfig:sdp_free} SDP in dB, \protect\subref{subfig:tir_free} TIR in dB and perceptual metrics of \protect\subref{subfig:stoi_free} STOI in a range of $0.0$ to $1.0$, and \protect\subref{subfig:psmt_free} PSMt in a range of $-1.0$ to $1.0$, respectively, are shown. AC was calculated zone-wise, whereas the rest of the metrics were calculated point-wise. Note that three different values for the number of eigenvectors in AP-VAST are denoted as APa (all eigenvectors), APh (half of the eigenvectors), APq (quarter of the eigenvectors). Besides, P-VAST using quarter of the eigenvectors is denoted as Pq, ACC-PM is denoted as ACM, and NC for without any control, respectively.}
		\label{fig:objresults_free_sim1}
\end{figure*}

==> chapters/04_simulations/ch4_0_sub2_sim1_reverb.tex <==
\begin{figure*}[t]
	\centering
	\captionsetup[subfigure]{justification=centering}
	    \subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim1_revb/fig_AC_(dB)_reverberant_pointwise.png}\label{subfig:ac_revb}}\quad
    	\subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim1_revb/fig_nSDP_(dB)_reverberant_pointwise.png}\label{subfig:sdp_revb}}\quad
		\subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim1_revb/fig_TIR_(dB)_reverberant_pointwise.png}\label{subfig:tir_revb}}
		
		\subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim1_revb/fig_STOI_reverberant_pointwise.png}\label{subfig:stoi_revb}}\quad
		\subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim1_revb/fig_PSMt_reverberant_pointwise.png}\label{subfig:psmt_revb}}
% 		\subfloat[]{\includegraphics[width=8.4cm]{data/figure_metric_TPS_nonadaptive_avg.png}\label{subfig:tps_revb}} , and \protect\subref{subfig:tps_revb} TPS
		\caption{\cc{The mean values (crosses) and the $95\%$ confidence intervals (solid lines) of the performance evaluation metrics in reverberant environment with $T_{60} = 200$ ms: physical metrics of \protect\subref{subfig:ac_revb} AC, \protect\subref{subfig:sdp_revb} SDP, \protect\subref{subfig:tir_revb} TIR and perceptual metrics of \protect\subref{subfig:stoi_revb} STOI, and \protect\subref{subfig:psmt_revb} PSMt are shown. AC was calculated zone-wise, whereas the rest of the metrics were calculated point-wise. Note that three different values for the number of eigenvectors in AP-VAST are denoted as APa (all eigenvectors), APh (half of the eigenvectors), APq (quarter of the eigenvectors). Besides, P-VAST using quarter eigenvectors is denoted as Pq, ACC-PM is denoted as ACM, and NC for without any control, respectively.}}
		\label{fig:objresults_revb_sim1}
\end{figure*}

==> chapters/04_simulations/ch4_0_sub2_sim2_reverb.tex <==
\begin{figure*}[t]
	\centering
	\captionsetup[subfigure]{justification=centering}
	    \subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim2/fig_AC_(dB)_reverberant_pointwise.png}\label{subfig:ac_revb_sim2}}\hfill
    	\subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim2/fig_SDP_(dB)_reverberant_pointwise.png}\label{subfig:sdp_revb_sim2}}\hfill
		\subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim2/fig_TIR_(dB)_reverberant_pointwise.png}\label{subfig:tir_revb_sim2}}\hfill
		
		\subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim2/fig_STOI_reverberant_pointwise.png}\label{subfig:stoi_revb_sim2}}\hfill
		\subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim2/fig_PSM_reverberant_pointwise.png}\label{subfig:psm_revb_sim2}}
		\hfill
		\subfloat[]{\includegraphics[width=5.8cm]{data/reverberant/sim2/fig_PSMt_reverberant_pointwise.png}\label{subfig:psmt_revb_sim2}}
		\caption{The mean values (crosses) and the $95\%$ confidence intervals (solid lines) of the performance evaluation metrics in reverberant environment ($T_{60} = 200$~ms) with respect to the length of the time segment $N$: physical metrics of \protect\subref{subfig:ac_revb_sim2} AC, \protect\subref{subfig:sdp_revb_sim2} SDP, \protect\subref{subfig:tir_revb_sim2} TIR and perceptual metrics of \protect\subref{subfig:stoi_revb_sim2} STOI, \protect\subref{subfig:psm_revb_sim2} PSM and \protect\subref{subfig:psmt_revb_sim2} PSMt are shown. AC was calculated zone-wise, whereas the rest of the metrics were calculated point-wise. The candidates of the segments length of durations $N$ are $60$~ms, $120$~ms, $500$~ms, $1000$~ms, and the input signal length which is plotted as \texttt{\scriptsize{all}}. Note that three different values for the number of eigenvectors in AP-VAST are denoted as APa (all eigenvectors), APh (half of the eigenvectors), APq (quarter of the eigenvectors). Besides, P-VAST using quarter of the eigenvectors is denoted as Pq, ACC-PM is denoted as ACM, and NC for without any control, respectively.}
		\label{fig:objresults_revb_sim2}
\end{figure*}
% We considered the segments length of durations $60\text{ ms, }120\text{ ms, }500\text{ ms, }1000\text{ ms}$, and the input signal length (i.e., $6.0$, $4.5$, and $4.0$ seconds, respectively)


==> chapters/04_simulations/ch4_2_opq_futurework.tex <==
\subsection{Open question and future work}
\label{ssec:limfut}

% \input{chapters/04_simulations/exp0/exp0_summary_ac.tex}

\input{chapters/04_simulations/exp0/exp0_summary_reprod_wrt_mu.tex}

% As seen in Fig.\ \ref{fig:exp0_ac_by_acc}, more than $20$ dB of the acoustic contrast with the given system geometry is achieved below $1$~kHz using the frequency domain ACC, and this is data-independent. From the optimization problem point of view, it is easier to achieve high acoustic contrast on a low frequency range rather than a high frequency range. 

When a large $\mu$ is used, AP-VAST seeks for the solution which provides high acoustic contrast over the signal distortion. This \ccs{can easily be} obtained when the signal distortion is allocated in the high frequency range; hence, this affects the result of AP-VAST with a large $\mu$ as if a low-pass filter is applied. As an example, the desired spectrum and the reproduced spectrum at the center of each zone are depicted in Fig.\ \ref{fig:exp0_reprod_wrt_mu}. The considered input signal is the English version of the dialogue from ``Zootopia'' in the anechoic environment. The averaged spectrum is computed with the frequency resolution of $66.67$~Hz after each segment without an overlap is windowed by the Hanning window. The maximum value is normalized to $0$~dB.

First, when $\mu = 1$, the spectrum of the reproduced signal in the bright zone follows the desired spectrum and that in the dark zone is lower especially in a low frequency range. Note that this is the case that the acoustic contrast and the signal distortion are equally important since $\mu = 1$. Large acoustic contrast is obtained at the range of frequency below $1$~kHz. When $\mu$ is large enough, large acoustic contrast is obtained at the frequency below $1$~kHz but at the cost of penalizing the spectrum in the high frequency range. This explains such a low-pass filter artifact when a large $\mu$ is chosen. Finding an optimal $\mu$ \ccs{as described in \cite{Liming2020}} for each segment \ccs{might alleviate this artifact.} %Large acoustic contrast is obtained at the range of frequency below $1$~kHz which we can see a similar trend in Fig.\ \ref{fig:exp0_ac_by_acc}.

==> chapters/04_simulations/definitions.tex <==
In this section, the performance of the proposed RR-CG method for sound zone control is compared with the VAST, ACC and PM methods on real speech signals. In Subsection \ref{sub:perfmeas}, we first define three types of performance measures to quantify the experimental results. The experimental results are presented in Subsection \ref{sub:expres}.
\subsection{Performance measures}
\label{sub:perfmeas}
Three performance measures are considered:

\noindent Acoustic contrast (AC): It is calculated based on the ratio of the signal powers of the reproduced sound in the bright zone and dark zone, i.e., 
\begin{align}
\text{AC} = 10 \log10\frac{\frac{1}{M^\text{B}}\sum_{m=1}^{M^\text{B}}\mathbf{E}{({y}_n^{m,\text{B}}})^2}{\frac{1}{M^\text{D}}\sum_{m=1}^{M^\text{D}}\mathbf{E}{({y}_n^{m,\text{D}}})^2},
\end{align}
where $\mathbf{E}(\cdot)$ is the expectation operator.

\noindent Signal distortion (SD): It is computed using the desired and reproduced sound signals in the bright zone, i.e.,
\begin{align}
\text{SD} = 10 \log10\frac{\sum_{m=1}^{M^\text{B}}\mathbf{E}{({d_n^{m,\text{B}}}-{y}_n^{m,\text{B}}})^2}{\sum_{m=1}^{M^\text{B}}\mathbf{E}{({d}_n^{m,\text{B}})^2}}.
\end{align}

\noindent Signal to interference ratio (SIR):  It is calculated based on the ratio of the signal powers of the reproduced sound and interference sound in the given zone, i.e., 
\begin{align}
\text{SIR} = 10 \log10\frac{\sum_{m=1}^{M^\text{B}}\mathbf{E}{({y}_n^{m,\text{B}}})^2}{\sum_{m=1}^{M^\text{B}}\mathbf{E}{({y}_{n,\text{inter}}^{m,\text{B}}})^2}.
\end{align}
where ${y}_{n,\text{inter}}^{m,\text{B}}$ denotes the interference sound in the given zone, and it is produced when this bright zone is treated as a dark zone for another input sound signal. Note that this metric is also known as the target-to-interferer ratio (TIR).

==> chapters/04_simulations/exp0/exp0_summary_ac.tex <==
\begin{figure}[t]
	\centering
    \input{chapters/04_simulations/exp0/exp0_ac_by_acc.tex}
	\caption{\cc{Acoustic contrast per frequency bin obtained by the frequency-domain ACC \cite{choi2002generation} after a regularization based on the truncated singular value decomposition (TSVD) described in \cite{Chang2012} being applied.}}
	\label{fig:exp0_ac_by_acc}
\end{figure}



==> chapters/04_simulations/exp0/exp0_summary_msk.tex <==
\begin{figure}[t]
	\centering
    \input{chapters/04_simulations/exp0/exp0_maskingcurves_every10th_half.tex}
	\caption{\cc{Masking curve of the speech signal for zone $\alpha$ in the first experiment from every $10$th segment (gray) and averaged across all the spectrums (black), respectively. In order to provide a better understanding, a masking curve (blue) calculated based on a segment which contains no signal and a masking curve (red) calculated based on a segment which contains speech are plotted, respectively.}}
% 	\label{fig:exp0_mskcurves}
\end{figure}


==> chapters/04_simulations/exp0/exp0_summary_reprod_wrt_mu.tex <==
\begin{figure}[t]
	\centering
    \input{chapters/04_simulations/exp0/exp0_reprod_wrt_mu.tex}
	\caption{\cc{The spectrum of the desired and reproduced signals at the center of the zones with a fixed $V = 1080$ for two different $\mu$: bright zone with $\mu=1$ (red solid), dark zone with $\mu=1$ (gray solid), bright zone with $\mu=100$ (blue solid), dark zone with $\mu=100$ (gray dash-dot), and the desired spectrum (gray solid thick).}} %Note that the considered input signal is the English version of the dialogue from ``Zootopia'' in the anechoic environment.}} %bright zone with $\mu=10$ (green solid), dark zone with $\mu=10$ (gray dash),
	\label{fig:exp0_reprod_wrt_mu}
\end{figure}



==> chapters/04_simulations/exp4/exp4_summary_org.tex <==
\begin{table*}[t]
\begin{threeparttable}
\caption{The Mean and the 95~\% Confidence Interval of the Performance Metrics of the Speech Signal for Zone $\beta$ in the Reverberant Environment}
\label{tab:exp4_pfmmtx}

\begin{tabular*}{2\columnwidth}{@{\extracolsep{\fill}} r c c r r r r r}
\toprule
     Method & \multicolumn{2}{c}{Parameter} & \multicolumn{5}{c}{Performance metric}\\ 
\cmidrule{2-3} 
    & \multicolumn{1}{c}{$1\leq V \leq 1920$} & \multicolumn{1}{c}{$\mu \geq 0$} & \multicolumn{1}{c}{AC (dB)} & \multicolumn{1}{c}{nSDP (dB)} & {TIR (dB)} & \multicolumn{1}{c}{STOI} & \multicolumn{1}{c}{PSMt}\\
\midrule
    No control & {NA\tnote{a}} & NA & -1.3 & 14.2 $\pm$ 0.5  & -0.1 $\pm$ 0.3 & 0.64 $\pm$ 0.004 & 0.14 $\pm$ 0.025\\
\addlinespace
    PM \cite{Simon-Galvez2015} & 1920 & 1.0 & 10.5 & \textbf{-9.9} $\pm$ \textbf{0.7} & 11.5 $\pm$ 0.5 & 0.80 $\pm$ 0.003 & 0.39 $\pm$ 0.009\\
    ACC \cite{choi2002generation} & NA & NA & 9.2 & 0.4 $\pm$ 0.8 & 9.3 $\pm$ 0.4 & 0.77 $\pm$ 0.013 & 0.40 $\pm$ 0.014\\
\addlinespace
    VAST \cite{Lee2018} & 1080 & 1.0 & 12.2 & -7.8 $\pm$ 0.7 & \textbf{12.8} $\pm$ \textbf{0.7} & 0.80 $\pm$ 0.004 & 0.43 $\pm$ 0.016\\
    P-VAST \cite{Lee2019} & 1080 & 1.0 & \textbf{14.9} & -7.2 $\pm$ 0.6 & 11.8 $\pm$ 0.6 & 0.76 $\pm$ 0.004 & 0.40 $\pm$ 0.022\\
\addlinespace
    AP-VAST & 1080 & 1.0 & 12.0 & -8.4 $\pm$ 0.4 & 12.2 $\pm$ 0.3 & \textbf{0.82} $\pm$ \textbf{0.004} & \textbf{0.54} $\pm$ \textbf{0.010}\\
\bottomrule
\end{tabular*}

\smallskip
\scriptsize
\begin{tablenotes}
\RaggedRight
\item[a] NA: Not applicable
\end{tablenotes}
\end{threeparttable}
\end{table*}
